RevDedup: A Reverse Deduplication Storage System Optimized for Reads to Latest Backups

Scaling up the backup storage for an ever-increasing volume of virtual machine (VM) images is a critical issue in virtualization environments. While deduplication is known to effectively eliminate duplicates for VM image storage, it also introduces fragmentation that will degrade read performance. We propose RevDedup, a deduplication system that optimizes reads to latest VM image backups using an idea called reverse deduplication. In contrast with conventional deduplication that removes duplicates from new data, RevDedup removes duplicates from old data, thereby shifting fragmentation to old data while keeping the layout of new data as sequential as possible. We evaluate our RevDedup prototype using microbenchmark and real-world workloads. For a 12-week span of real-world VM images from 160 users, RevDedup achieves high deduplication efficiency with around 97% of saving, and high backup and read throughput on the order of 1GB/s. RevDedup also incurs small metadata overhead in backup/read operations.

==> challenges.tex <==
\section{Background and Motivation}
\label{sec:background}

Deduplication is a well-known technique for exploiting content similarities
and eliminating the storage of redundant data.  Typical deduplication systems
divide a backup stream into {\em blocks}, and use {\em fingerprints} to
identify blocks and check if blocks can be deduplicated.  A fingerprint is
computed by a cryptographic hash (e.g., MD5, SHA-1) of the content of a block.
Two blocks are said to be identical if their fingerprints are the same. We
assume that the probability that two different blocks have fingerprint
collisions is negligible \cite{black06}.  Deduplication has been widely used
in backup applications (see \S\ref{sec:related}).  
%Existing deduplication studies mainly focus on improving storage efficiency,
%memory usage, or write performance.  However, deduplication significantly
%degrades read performance due to fragmentation.
In the following, we overview the challenges of building a deduplication
system for backup storage. 

%In particular, several studies show the effectiveness of applying
%deduplication to virtual machine (VM) image backup storage, due to the large
%content similarities among VM images
%\cite{clements09,jayaram11,jin09,liguori08,ng11,rhea08}.  
%the fragmentation problem.  Then we state our design goals of building a
%deduplication system for VM image backup storage. 

%\subsection{Challenges}
%\label{subsec:challenges}

{\bf Storage efficiency.} Prior studies (e.g., \cite{rhea08,zhu08}) strive to
maximize disk space saving by fully eliminating all duplicate blocks.  More
recent studies (e.g.,
\cite{bhagwat09,elshimi12,guo11,kruus10,lillibridge09,srinivasan12}) propose
to trade storage efficiency for deduplication performance.  That is, by
allowing the storage of few duplicate blocks, the duplication performance can
be remarkably improved.  It is important to keep the number of duplicate
blocks minimal, so that the storage efficiency is comparable to the full
deduplication systems \cite{rhea08,zhu08}. 

{\bf Memory usage for indexing.}  Since the number of fingerprints increases
proportionally with the raw storage size,  it is infeasible to keep all
fingerprints and other indexing metadata in main memory.  Thus, some indexing
metadata must be kept on disk. This introduces disk accesses and degrades the
deduplication performance.  Some studies (e.g., 
\cite{bhagwat09,kruus10,lillibridge09,xia11,zhu08}) exploit similarity and
locality characteristics of backup streams to minimize the disk accesses for
fingerprint lookups.  In general, it is important to balance the memory usage
and the indexing performance. 

%However in handling duplicates across different backup streams, there is no
%characteristics to follow. 

{\bf Write performance.} The write performance of a deduplication system is
determined by several factors: fingerprint computations, fingerprint lookups,
metadata updates, and disk writes.  Minimizing their overheads is important
for high write performance.  In distributed backup systems (e.g.,
\cite{guo11}), the network transfer overhead of transmitting backup data
should also be minimized.  Most inline deduplication systems enjoy large
speedup in backup systems by eliminating the writes of duplicate content.
However, if the backup stream contains unique data without any duplicates, 
then the write throughput of a deduplication system should be comparable to
the raw disk write throughput achievable by traditional storage systems
without deduplication.

% system is critical as it determines the number of VM instances that the system
% can serve in a specific amount of time. Most deduplication system enjoys large
% speedup by discarding write on duplicated contents. Yet we believe that this
% speedup is largely determined by the user behavior on the image, and therfore
% it should not become the performance target of the system. Instead the main
% focus should be whether the deduplication process in the write path slows down
% the write throughput, and whether the maximal raw write throughput of the
% disks can be achieved.

% \noindent{\bf Bandwidth.} For backup systems, there is usually a dedicated
% link, for example, a fibre-channel, between the primary server and the backup
% system.  Such a physical link provides best insulation of backup process to
% primary workloads. Nonetheless in virtualization platforms, the link between
% the backup server and the VM hosts are usually shared with the operational
% network, in which virtual machines are using for primary purpose. Therefore
% the system should try to minimize network transfer whenever possible, so that
% primary operations are no disrupted by the backup process.

%Deduplication enabled backup systems usually follow a traditional approach:
%in order to minimize the backup window and increase the write throughput,
%duplicated data are discarded in the write path, and the system instead
%creates a smaller-size references to some data already stored in the
%disk. However, as each backup has some unique contents, this approach
%generates a side effect that cannot be unwinded: data fragmentation, and
%reduces the read throughput dramatically when the backup is useful.

{\bf Read performance.}  Most deduplication systems suffer from the
inherent fragmentation problem, which has also been addressed in prior work
\cite{kaczmarczyk12,rhea08,srinivasan12}.  We now illustrate the
fragmentation problem using a simple example. 
Figure~\ref{fig:eg_trad}(a) shows that a deduplication system is about to
write, in order, three snapshots of a VM, denoted by VM$_1$, VM$_2$, and
VM$_3$.  We assume that each VM image has eight blocks, and that the system
has no data initially.  Figure~\ref{fig:eg_trad}(b) shows how a traditional
deduplication system writes data.  First, the system writes VM$_1$ with unique
blocks {\sf A} to {\sf H}.  Given that all blocks are new, the system will
sequentially write all of them into disk.  Next, the system writes VM$_2$, in
which some of the blocks are identical to those of VM$_1$. Then the system
stores only the smaller-size references to refer to those identical blocks,
and appends the unique blocks {\sf D'} and {\sf F'} to the end of the last
write position.  The same approach applies when the system writes VM$_3$, and
it only writes the unique blocks {\sf E'}, {\sf F''}, and {\sf H'} to the end
of the last write position.  
\begin{comment}
\begin{figure*}[t]
\centering
\begin{tabular}{c@{\ }c@{\ }c}
\includegraphics[width=0.9in,angle=270]{figs/eg_a} &
\includegraphics[width=0.9in,angle=270]{figs/eg_b} &
\includegraphics[width=0.9in,angle=270]{figs/eg_c}
\vspace{6pt}\\
\mbox{(a) Backups} &
\mbox{(b) Conventional deduplication} &
\mbox{(c) RevDedup}
\end{tabular}
\vspace{-6pt}
\caption{An example of how conventional deduplication and RevDedup place data
on disk.}
\label{fig:eg_trad}
\end{figure*}
\end{comment}

\begin{figure*}[t]
\centering
\begin{minipage}{0.205\linewidth}
\centering
\includegraphics[width=\linewidth]{eg_am}
\mbox{(a) Backups}
\end{minipage}%
\hspace{3pt}
\begin{minipage}{0.36\linewidth}
\centering
\includegraphics[width=\linewidth]{eg_bm}
\mbox{(b) Conventional deduplication}
\end{minipage}%
\hspace{3pt}
\begin{minipage}{0.39\linewidth}
\centering
\includegraphics[width=\linewidth]{eg_cm}
\mbox{(c) RevDedup}
\end{minipage}%
\caption{An example of how conventional deduplication and RevDedup place data
on disk.}
\label{fig:eg_trad}
\end{figure*}
%
%\begin{figure}[t]
%\centering
%\includegraphics[height=\linewidth,angle=270]{figs/eg_timededup}
%\caption{An example of how a RevDedup places data on disk.}
%\label{fig:eg_timededup}
%\end{figure}

From Figure~\ref{fig:eg_trad}(b), we see that the blocks of the newly written
VM image are re-ordered and randomly scattered throughout the disk.  Reading
VM$_3$ generates many disk seeks and significantly lowers the read
performance.  We can perform simple calculation to understand the degradation
due to disk seeks.  Consider a generic 7200~RPM 3.5-inch SATA harddisk with an
average seek time of 8.5ms \cite{seagate}.  With only 60 disk seeks per second
in the read path, the read throughput can drop by at least 50\% compared to
the sequential read (which we assume has negligible seek time). 

% We can use some citations to prove deduplication can cause > 50\% drop in read
Although backup data is less frequently read than other interactive
applications, maintaining high read performance for deduplication backup
systems is necessary.  For disaster recovery, minimizing the time of restoring
all backups implies that the system downtime is minimized.  Also, high read
performance makes new applications feasible.  For example, administrators can
retrieve recent backup VM images to conduct forensics analysis. 

Our observation is that the latest backup contain the ``hot'' data and are
expected to be more likely read in practice, while older backups contain
``cold'' data that usually serves the compliance purpose and
should be seldom read.   This guides our design of RevDedup.
Figure~\ref{fig:eg_trad}(c) shows the disk layout for the previous example
when RevDedup is used.  We allow the blocks of VM$_3$ (i.e., the latest
backup) to be sequentially placed on disk.  Also, the blocks of VM$_2$ are
less fragmented than VM$_1$ (i.e., the blocks are less spread out on disk).
Thus, the newer a backup version is, the less fragmentation overhead the
backup will experience.  We explain in detail how we achieve this property in
\S\ref{sec:design}. 
	
%\subsection{Challenges}
%\label{subsec:challenges}

% Most of the existing deduplication systems are designed exclusively for
% backing up a few specific servers. The assumptions about the system
% environment may not be applicable to a virtualization platform running
% multiple virtual machines in a number of VM hosts. In the following, we list
% out the challenges in designing a deduplication system for a virtualization
% platform with a large number of virtual machines.

% It is virtually impossible for having a raw disk read throughput for all
% backups, as deduplication causes data fragmentation. However not all backups
% are subject to reads in the future. For example backups older than one year
% should have a lower read opportunity than backups in a few days. Therefore by
% considering the system's overall performance, the read throughput of recent
% backups should match the match the raw disk throughput, while the patience on
% read aged backups can be greater.


==> implementation.tex <==
%\subsection{Implementation Details}
%\label{subsec:implementation}
%
%Our RevDedup prototype is mainly implemented in C on Linux. Both the segment and
%block fingerprints we used in RevDedup is SHA-1. We now elaborate its
%implementation details.
%
%{\bf Storage backend.} The RevDedup server mounts its data storage backend 
%on a native file system.  RevDedup requires that the file system support the
%hole-punching operation.  Examples of such file systems include Ext4 and XFS
%on Linux.
%
%{\bf Client-server communication.} The client-server communication of RevDedup
%is based on the RESTful web API, which is built on HTTP. The server uses GNU
%{\tt libmicrohttpd} \cite{libmicrohttpd} as the HTTP server frontend, while each
%client uses {\tt libcurl} \cite{libcurl} to generate HTTP requests. All
%client-server communications are stateless.  The server can process multiple
%requests simultaneously without any locking. Also since RevDedup server exposes
%RESTful APIs, any client complying with RevDedup's communication protocol can
%perform backup and restore operations.  For example, a client can simply use a
%lightweight Linux program {\tt wget} to retrieve a VM image using the correct
%URI request.
%
%{\bf Handling of null blocks.} 
%In practice, VM images contain a large number of null (or zero-filled) blocks
%\cite{jin09}.  In RevDedup, the server skips the writes of any null blocks
%presented in the segments submitted by a client.  When a null block is to be
%read, the server generates null data on the fly instead of reading it from
%disk.
%
%{\bf Multi-threading.} We extensively leverage multi-core technologies in
%RevDedup. In writes, we use multiple threads to receive segment uploads from
%the clients and  compare block fingerprints in segment rebuilding. For
%reads, we use dedicated threads to pre-declare the segment reads in kernel by using the
%POSIX function {\tt posix\_fadvise(POSIX\_FADV\_WILLNEED)}. With the
%pre-declaration of the read pattern, the kernel can make effective pre-fetching
%of segments, and hence improve the read performance. Also we use a separate
%thread for merging the reference chains of blocks in an earlier backup version.
%Once a particular block address is rebuilt, the thread pushes the address to the
%main thread. Thus the main thread does not need to wait for the completition of
%all reference chains, resulting an improved read performance. We compare the
%time required to rebuild the reference chains and to read the backup versions in
%Section~\ref{sec:evaluation}.


==> related.tex <==
%\section{Related Work}
%\label{sec:related}
%
%%Existing studies on deduplication mainly target backup systems.  
%%It has been shown to be effective in
%%reducing storage for VM images \cite{jayaram11,jin09,liguori08,nath06}.  In
%%this section, we review related work on improving the performance of
%%deduplication storage systems. 
%
%We review related work on deduplication storage. 
%
%{\bf Deduplication for backup storage.} Most existing deduplication studies
%for backup storage focus on optimizing fingerprint indexing to achieve high
%backup performance.  Deduplication is first proposed in Venti \cite{quinlan02}
%for data backup in content-addressable storage systems.  DDFS \cite{zhu08} and
%Foundation \cite{rhea08} use compact data structures to minimize memory usage
%for indexing.  DDFS further exploits spatial locality to cache the
%fingerprints of blocks that are likely accessed later.  Other studies
%\cite{lillibridge09,bhagwat09,kruus10,guo11,xia11} exploit workload
%similarities to reduce memory usage. 
% 
%%keeps only small portions of index samples in memory by exploiting chunk
%%locality, such that the chunk orders of different backup streams are likely
%%preserved.  
%%exploits file similarity of backup streams, and keeps only a 
%%representative fingerprint per file in memory.  A similarity signature scheme
%%is proposed in \cite{aronovich09} to identify similar large-size chunks for
%%deduplication.  Bimodal \cite{kruus10} reduces memory usage via different
%%granularities of backup regions.  ChunkStash \cite{debnath10} and Dedupv1
%%\cite{meister10} use solid state drives (SSDs) to store fingerprints.  The
%%fast random I/Os of SSDs enable high-performance deduplication compared to the
%%solutions based on memory and disk only.  Guo {\em et al.} \cite{guo11}
%%propose sampled indexing and trades storage efficiency for less memory usage,
%%and pipelined implementation to increase the backup throughput.  We point
%%out that \cite{guo11} also experiments the read performance using their
%%deduplication design, but it does not provide any solution that
%%specifically optimizes the read performance.  Silo \cite{xia11} improves
%%Extreme Binning \cite{bhagwat09} by packing small files into larger segments.
%
%The above studies aim to achieve high write throughput and high storage
%efficiency, but put limited emphasis on read performance.  Guo {\em et al.}
%\cite{guo11} also experiment the read performance of their deduplication
%prototype, but they do not provide any explicit solution that optimizes reads. 
%Similar to our work, Kaczmarczyk {\em et al.} \cite{kaczmarczyk12} also
%improve read performance for latest backups in deduplication.  Their system
%selectively rewrites deduplicated data to disk to mitigate fragmentation, and
%removes old rewritten blocks in the background.  However, they consider
%deduplication for different versions of a single backup only, while we enable
%global deduplication across multiple VM backups.  Nam {\em et al.} \cite{nam12}
%measure the fragmentation impact given the input workload and activates
%selective deduplication on demand.  Note that both studies
%\cite{kaczmarczyk12,nam12} only conduct simulation-based evaluations, while we
%implement a prototype to experiment the actual I/O throughput.
%
%{\bf Distributed deduplication.} DeDe \cite{clements09} targets a storage area
%network (SAN) connecting multiple client hosts that run VM instances.  It
%performs out-of-order deduplication in the hosts to minimize the
%synchronization overhead.  Our work also considers multiple clients, 
%yet we assume only standard Gigabit Ethernet connections and we focus on
%inline deduplication.  HYDRAstor \cite{dubnicki09} and its successor HydraFS
%\cite{ungureanu10} are distributed deduplication systems with multiple storage
%nodes. Our work focuses on a single storage backend. 
%
%{\bf Deduplication for primary storage.} In addition to backup systems,
%several file systems (e.g., \cite{lessfs,ng11,opendedup,zfs}) deploy inline
%deduplication. iDedup \cite{srinivasan12} is a primary, inline deduplication
%systsem system that optimizes read performance.  It applies deduplication to
%chains of duplicate 4KB blocks of some predefined length. For each block to be
%written, it searches for all candidate block chains containing the block and
%identifies the longest duplicate block chain for deduplication. However, the
%search of block chains can become a bottleneck if there are many candidate
%chunk sequences.  It also does not optimize reads specifically for latest data
%as in our work.  Windows Server deploys a primary deduplication file system
%\cite{elshimi12} that exploits data compression to maintain high storage
%efficiency with a large block size being used for deduplication. 
%
%%{\bf Mitigating fragmentation.} Most deduplication storage systems suffer
%%fragmentation, as pointed out in \cite{rhea08}. To mitigate fragmentation, 
%%iDedup \cite{srinivasan12} deduplicates only a sequence of duplicate blocks
%%whose length is larger than a predefined threshold, and amortizes the disk
%%seeks in block reads.  A closely related work to ours is \cite{kaczmarczyk12},
%%which proposes a backup system that mitigates fragmentation for more recent
%%backups. Its idea is to selectively rewrite some deduplicated data into the
%%disk, so as to reduce random I/Os in subsequent reads.  It uses a background
%%process to remove old rewritten blocks.  Note that \cite{kaczmarczyk12} only
%%focuses on mitigating fragmentation of different versions of the same backup
%%stream, and does not consider deduplication across backup streams.  Also,
%%\cite{kaczmarczyk12} only focuses on a single-disk system, and its scalability
%%toward a disk-array system remains open. 
%
%{\bf Version control systems.} Our work in essence provides similar
%functionalities as in traditional version control systems.  Rdiff-backup
%\cite{rdiffbackup} and Subversion \cite{svn} generate changes between adjacent
%versions on a per-file basis.  In particular, Subversion improves restore
%performance via a skip-list data structure.  Note that both studies do not
%address global deduplication as in our work.  Git \cite{git} enables global
%deduplication, but only in the whole-file level rather than more the more
%fine-grained block level. 
%%rdiff-backup, subversion cannot perform global deduplication. 
%%. Each file has a
%%unique fingerprint generated by its content.  If two files have identical
%%content, then only one copy is stored.  However, it uses file-level
%%deduplication only, and stores the entire file if it has been modified. It
%%generally uses more storage space. 
%%by only storing deltas (i.e. changes) of between versions of a file. Deltas can
%%be backward-pointing or forward pointing. 
%
%%\cite{loeliger09}, and generally requires more storage space.
%
%
%%Oracle ZFS \cite{zfs}, Opendedup SDFS \cite{opendedup}, lessfs \cite{lessfs} and
%%LiveDFS \cite{ng11} are primary file systems that support inline deduplication.
%%ZFS targets enterprise-scale systems, and is built for the Oracle Solaris
%%platform. Opendedup SDFS is an open-source deduplication file system which
%%places all the fingerprints in memory to provide fast fingerprint lookup.
%%lessfs, in contrast, outsources fingerprint management by a dedicated database
%%engine. LiveDFS is another deduplication file system mainly designed for VM
%%image storage. It maintains a compact memory index, and exploits locality for
%%storing fingerprints in disk. Microsoft also developed a primary deduplication
%%file system \cite{elshimi12}. It exploits data compression so that the system
%%can achieve the same storage efficiency with a larger block size for
%%deduplication, and partitions data so as to reduce the index size in memory.
%
%%\smallskip\noindent {\bf VM image storage and backup.} Liguori {\em et al.} and
%%Jin {\em et al.} \cite{liguori08, jin09} have shown that deduplication can
%%significantly enhance storage efficiency for VM images. Nath {\em et al.}
%%\cite{nath06} evaluate a deployed CAS system for storing VM images, and focus on
%%storage efficiency and network load. Liguori {\em et al.} \cite{liguori08}
%%deploy a CAS system based on Venti \cite{quinlan02} for storing VM images.
%%LiveDFS \cite{ng11} mainly focuses on storing the master VM image in the cloud,
%%and does not consider storing backups of VM instances. CloudVS \cite{tang12}
%%propose a version control system for virtual machines. It applies technique in
%%redundancy elimination to minimize the network transfer and storage overhead.
%
%% For software project repositories, the redundent storage spaces is small as
%% Git usually tracks program codes. However, the content addressable storage
%% solution cannot be applied to VM backup storage.
%

